Contextual Active Model Selection

While training models and labeling data are resource-intensive, a wealth of pre-trained models and unlabeled data exists. To effectively utilize these resources, we present an approach to actively select pre-trained models while minimizing labeling costs. We frame this as an online contextual active model selection problem: At each round, the learner receives an unlabeled data point as a context. The objective is to adaptively select the best model to make a prediction while limiting label requests. To tackle this problem, we propose CAMS, a contextual active model selection algorithm that relies on two novel components: (1) a contextual model selection mechanism, which leverages context information to make informed decisions about which model is likely to perform best for a given context, and (2) an active query component, which strategically chooses when to request labels for data points, minimizing the overall labeling cost. We provide rigorous theoretical analysis for the regret and query complexity under both adversarial and stochastic settings. Furthermore, we demonstrate the effectiveness of our algorithm on a diverse collection of benchmark classification tasks. Notably, CAMS requires substantially less labeling effort (less than 10%) compared to existing methods on CIFAR10 and DRIFT benchmarks, while achieving similar or better accuracy. Our code is publicly available at: https://github.com/xuefeng-cs/Contextual-Active-Model-Selection.

==> supp_hyperparameter.tex <==
\subsection{Hyperparameters}\label{app:Hyperparameters}

We performed our experiments on a Linux server with 80 Intel(R) Xeon(R) Gold 6148 CPU @ 2.40GHz and total 528 Gigabyte memory.

By considering the resource of server, We set 100 realizations and 3000 stream-size for DRIFT, 20 realizations and 10000 stream-size for CIFAR10, 200 realizations and 4000 stream size for HIV, 300 realization and 80 stream-size for VERTEBRAL. In each realization, we randomly selected steam-size aligned data from testing-set and make it as online streaming data which is the input of each algorithm. Thus, we got independent result for each realization. 

A small realization number would increase the variance of the results due to the randomness of stream order. A large realization number would make the result be more stable but at the cost of increasing computational cost (time, memory, etc.). We chose the realization number by balancing both aspects. 

\clearpage

==> supp_miscellaneous.tex <==
\clearpage
\section{\fix{Miscellaneous}}
















\subsection{How tight is the bound for query complexity in practice?}
We observe (in \figref{fig:exp:results}, Middle plots) that the query complexity grows sublinear in $T$. Although we do not have tightness results of the query complexity bounds, the proofs of  \thmref{thm:stochastic-query-complexity} and \thmref{thm:adversarial-query-complexity} are built on top of the regret bounds. In our revision, we have added to 
\secref{sec:analysis} (Theoretical Analysis) that our regret bounds in both stochastic settings and adversarial settings are tight up to a constant factor of existing lower bounds. We acknowledge that it is non-trivial to come up with a query complexity lower bound, and leave it as an interesting direction for future work.









==> supp_proofs_for_vc_dim.tex <==
\clearpage
\section{Theoretical Results for Infinite Policy Class (Finite VC Dimension)}\label{sec:app:analysis:infinite}

Next, for learning from multiple policies problem, there is one challenge that the size of the policy class $|\Policies|$ could be extremely large or infinite. 
In this section, we focus on the adversarial setting, and consider infinite policy classes with a finite VC dimension. 



Let us define the Vapnik-Chervnonenkis (VC) dimension of a hypothesis class $H$ as $\mathrm{VCdim}(H)$. $\mathrm{VCdim}(H)=\max{\paren{m\in N \mid \Pi_H\paren{m}=2^m}}$, which is the cardinality of the largest set of points in $X$ that can be shattered by hypothesis class $H$. We named the new algorithm $\algname_{\mathrm{VC}}$. Since it is in a standard VC-dimension definition, we assume we have only two base classifiers $\ModelsNum=2$. \citep{beygelzimer2011contextual} Here we only discussed the VC dimension for two actions/ classifiers. For multi-dimension, we could extend it by the Natarajan dimension.

We sketch our analysis framework below and provide the detailed analysis in the following subsections. $\algname_{\mathrm{VC}}$ first partitions the policy class $\Policies$ into equivalent classes based on each policy's sequential predictions at the first $\tau$ rounds. $\tau$ bounds the regret. Then it constructs a finite policy set $\Policies^{'}$ by picking a single policy from each class and testing \algname by using $\Policies^{'}$ on the rest $T-\tau$ rounds. By Sauer's lemma, we have $|\Policies^{'}|\leq \paren{\frac{e{\tau}}{d}}^d$. Combining it with \thmref{thm:adversarial-regret-bound},  we can get the regret bound of $\Loss_{\algname}\paren{\Policies^{'},T-\tau}$. Then we bound the regret of using policy set $\Policies^{'}$ to $\Policies$. We define the number of disagreement on the $T-\tau$ sequence as  $m = m\paren{\policy,\policy^{'}}$. Then we bound the agreement probability for size $\tau$ subset by $e^{-\frac{m\tau}{T}}$. Since there are $\paren{\frac{eT}{d}}^{2d}$ possible distinct pairs between $\Pi$ and $\Pi'$, we apply the union bound over every pair of policies. %
Finally, we reach the regret bound by combining the regret bounds from the above three parts.


\subsection{Regret bound} \label{app:vc_regret}
We formally state the regret bound for the infinite policy class setting as follows.




\begin{theorem}{(Regret)}\label{thm:vc-regret-bound}.
For any distributions over contexts and rewards, for all sets of policies $\Policies$ with VC dimension d, with probability $1-\frac{\delta}{2}$,
\[\mathcal{R}_T\paren{\algname}\leq
\paren{2|\domClabel|\sqrt{\ln{|\domClabel|}}+2}{{\sqrt{{T\cdot \paren{2d\ln{\frac{eT}{d}}+\ln{\frac{2}{\delta}}}}/{\fixremoved{\max}\{\minpgap{T},\fixremoved{\sqrt{1/T}}\}}}}}.
\]
\end{theorem}

The full proof for \thmref{thm:vc-regret-bound} 
is built upon \thmref{thm:adversarial-regret-bound}, while the proof structure depends on  \cite{beygelzimer2011contextual}.  %

\begin{proof}%

At the first $\tau$ rounds, the regret is bounded by $\tau$. In the following, we first bound the regret of \algname to policy set $\Policies^{'}$ for the remaining $T-\tau$ rounds, then we bound the regret of $\Policies^{'}$ to full policy set $\Policies$. 
In the end, we optimize with respect to the value of $\tau$ to achieve the result.

\emph{\underline{Step 1.} Bounding the regret of $\Loss_{\algname}\paren{\Policies^{'},T-\tau}:$}

Let us define $L_{\min}\paren{\Policies}$ as the return of the best policy in policy set $\Policies$ over T steps. By applying Sauer's lemma, we have $|\Policies^{'}|\leq \paren{\frac{e{\tau}}{d}}^d$, we can bound $\Loss_{\algname}\paren{\Policies^{'},T-\tau}$ with result from \thmref{thm:adversarial-regret-bound} by
\[
\Loss_{\algname}\paren{\Policies^{'},T-\tau} \leq \Loss_{\min{\paren{\Policies^{'}}}} + 2|\domClabel|\sqrt{\ln{|\domClabel|}}{\sqrt{\frac{\paren{T-\tau}\paren{d\ln{\frac{e\tau}{d}}}}{\fixremoved{\max}\{\minpgap{T-\tau},\fixremoved{\sqrt{1/{(T-\tau)}}}\}}}}.
\]

\emph{\underline{Step 2.} Bounding the regret of $\Policies^{'}$ to $\Policies:$ \\}
Sauer's Lemma implies the number of unique policies for any sequence of feature observations of context $x_1,...,x_T$ is bounded by $\paren{\frac{eT}{d}}^d$. Let us randomly pick subset $S$ of size $\tau$ of contexts and bound the probability that two policy $\pi$ and $\pi'$ agree on the subset. Let us defines the number of disagreement on the T-length sequence as $m = m\paren{\policy,\policy^{'}}$. Then

\[
\Prover{S}{\forall{x} \in S , \pi{\paren{x}}=\pi'{\paren{x}}}=\paren{1-\frac{m}{T}}^{\tau} \leq e^{-\frac{m\tau}{T}}\leq \delta_{0}
\]

Thus for any pair of $\policy,\policy' \in \Policies$ with $m\paren{\pi,\pi'}\geq \frac{T}{\tau}\ln{\frac{1}{\delta_{0}}}$, we 
have $Pr_S[\forall{x}\in S,\pi\paren{x}=\pi'\paren{x}]\leq \delta_{0}$. Since there are possible $\paren{\frac{eT}{d}}^{2d}$ distinct pairs between $\Pi$ and $\Pi'$.

We can get $\sum_{\Pi,\Pi'}\Pr{A\paren{\Pi,\Pi'}}\leq\paren{\frac{eT}{d}}^{2d}\delta_0$, 

\begin{flalign*}
\Pr{\bigcup_{\Pi,\Pi'}A\paren{\Pi,\Pi'}}\leq \sum_{\Pi,\Pi'}Pr\paren{A\paren{\Pi,\Pi'}} \leq\paren{\frac{eT}{d}}^{2d}\delta_0.
\end{flalign*}

Let us assume $\paren{\frac{eT}{d}}^{2d}\delta_0=\frac{\delta}{2}$, thus we get $\delta_0=\frac{\delta}{2}\paren{\frac{d}{eT}}^{2d}$. Since we have $m\paren{\pi,\pi'}\geq \frac{T}{\tau}\ln{\frac{1}{\delta_{0}}}$. 
By applying a union bound over every pair of policies, we get
\[
\Prover{S}{\exists \pi,\pi' , s.t. m\paren{\pi,\pi'} \geq \frac{T}{\tau}\paren{2d\ln\frac{eT}{d}+\ln{\frac{2}{\delta}}}}, 
\]
\[
s.t. {\forall{x}\in S,\pi\paren{x} = \pi'\paren{x}}\leq \frac{\delta}{2}.
\]

Hence, with probability $1-\frac{\delta}{2}$, we can get the following equation for any T-length sequences over a random subset of size $\tau$

\[
L_{\min}\paren{\Policies'}\leq L_{\min}\paren{\Policies} + \frac{T}{\tau}\paren{2d\ln\frac{eT}{d}+\ln{\frac{2}{\delta}}},
\]

Since the first $\tau$ samples of subset are from $i.i.d$ distribution and it is exchangeable. What's more, the above sequence holds for any T-length sequence. Consequently, with probability $1-\frac{\delta}{2}$, we have \\


\begin{flalign*}
\Loss_{\algname_{VC}} &\leq L_{\min}\paren{\Policies}+\tau +\frac{T}{\tau}\paren{2d\ln\frac{eT}{d}+\ln{\frac{2}{\delta}}} +2|\domClabel|\sqrt{\ln{|\domClabel|}}{\sqrt{\frac{\paren{T-\tau}\paren{d\ln{\frac{e\tau}{d}}}}{{\fixremoved{\max}\{\minpgap{T-\tau},\fixremoved{\sqrt{1/{(T-\tau)}}}\}}}}}\\
&\leq L_{\min}\paren{\Policies} +\tau +\frac{T}{\tau{\fixremoved{\max}\{\minpgap{T},\fixremoved{\sqrt{1/{T}}}\}}}\paren{2d\ln\frac{eT}{d}+\ln{\frac{2}{\delta}}} +2|\domClabel|\sqrt{\ln{|\domClabel|}}{\sqrt{\frac{T\cdot \paren{2d\ln{\frac{eT}{d}}+\ln{\frac{2}{\delta}}}}{{\fixremoved{\max}\{\minpgap{T},\fixremoved{\sqrt{1/{T}}}\}}}}}.
\end{flalign*}



\emph{\underline{Step 3.} Optimizing over $\tau$.} 

Let $\tau = {\sqrt{\frac{T\cdot \paren{2d\ln{\frac{eT}{d}}+\ln{\frac{2}{\delta}}}}{{\fixremoved{\max}\{\minpgap{T},\fixremoved{\sqrt{1/{T}}}\}}}}}$. We get

\begin{align*}
\Loss_{\algname_{\mathrm{VC}}} &\leq L_{\min}\paren{\Policies} + \paren{2|\domClabel|\sqrt{\ln{|\domClabel|}}+2}{{\sqrt{\frac{T\cdot \paren{2d\ln{\frac{eT}{d}}+\ln{\frac{2}{\delta}}}}{{\fixremoved{\max}\{\minpgap{T},\fixremoved{\sqrt{1/{T}}}\}}}}}}\\
&\stackrel{\paren{a}}{\leq} \tilde{\Loss}_{T,*} + \paren{2|\domClabel|\sqrt{\ln{|\domClabel|}}+2}{{\sqrt{\frac{T\cdot \paren{2d\ln{\frac{eT}{d}}+\ln{\frac{2}{\delta}}}}{{\fixremoved{\max}\{\minpgap{T},\fixremoved{\sqrt{1/{T}}}\}}}}}},
\end{align*}
where step (a) is by replacing $L_{\min}\paren{\Policies}= \tilde{\Loss}_{T,*}$.








\end{proof}




\subsection{Query complexity bound} 
\label{app:vc_query_complexity}

By following the proof of \thmref{thm:stochastic-query-complexity} and adapting the regret bound of \thmref{thm:vc-regret-bound}, we prove the sub-linear query complexity for the infinite policy class setting as follows. %
\begin{theorem}{(Query Complexity, informal)}\label{thm:vc-query-complexity}. Assume at least two models disagree at each round in a $|\domClabel|$ classification problem and assume for all sets of policies $\Policies$ with VC dimension $d$. For T $\geq$ 0, the expected query number till round T under VC Dimension setting with probability $1-\delta$ is at most
\[
{O}\paren{
\frac{{\ln\paren{T}}}{|\domClabel|\ln{|\domClabel|}}\paren{{{\sqrt{\frac{T\cdot \paren{2d\ln{\frac{eT}{d}}+\ln{\frac{2}{\delta}}}}{\fixremoved{\max}\{\minpgap{T},\fixremoved{\sqrt{1/T}}\}}}}}+\tilde{\Loss}_{T,*}}}.
\]
\end{theorem}

\begin{proof}%
From \lemref{lem:query_complexity}, we get the following equation as the cumulative query cost
\[
\expct{\sum_{t=1}^TU_t} \leq
\expct{\sum_{t=1}^T{\paren{\frac{1}{\sqrt{t}}+\frac{\sum_{y\in \domClabel} \langle \ModelsDistB_t,\lossB_t^y \rangle \log_{|\domClabel|}{\frac{1}{\langle \ModelsDistB_t,\lossB_t^y \rangle}}}{|\domClabel|}}}}.
\]

Let us assume the expected total loss of best policy is $\tilde{\Loss}_{T,*}$, thus from $\thmref{thm:vc-regret-bound}$, we get 

\[
    \expct{R_T}=\expct{\sum_{t=1}^T r_t}\leq \paren{2|\domClabel|\sqrt{\ln{|\domClabel|}}+2}{{\sqrt{\frac{T\cdot \paren{2d\ln{\frac{eT}{d}}+\ln{\frac{2}{\delta}}}}{{\fixremoved{\max}\{\minpgap{T},\fixremoved{\sqrt{1/{T}}}\}}}}}} + \tilde{\Loss}_{T,*}.
\]


By using \eqnref{eq:budget-eq}, we can get the following query complexity theory.
\begin{flalign*}
\expct{\sum_{t=1}^TU_t}&\leq 2\sqrt{T}+\\
&\frac{\paren{ \paren{2|\domClabel|\sqrt{\ln{|\domClabel|}}+2}{{\sqrt{\frac{T\cdot \paren{2d\ln{\frac{eT}{d}}+\ln{\frac{2}{\delta}}}}{{\fixremoved{\max}\{\minpgap{T},\fixremoved{\sqrt{1/{T}}}\}}}}}}+\tilde{\Loss}_{T,*}}\paren{\log_{|\domClabel|}\frac{T^2\paren{|\domClabel|-1}}{\paren{ \paren{2|\domClabel|\sqrt{\ln{|\domClabel|}}+1}{{\sqrt{\frac{T\cdot \paren{2d\ln{\frac{eT}{d}}+\ln{\frac{2}{\delta}}}}{{\fixremoved{\max}\{\minpgap{T},\fixremoved{\sqrt{1/{T}}}\}}}}}}+\tilde{\Loss}_{T,*}}^2}}}{|\domClabel|}\\
&\leq 2\sqrt{T}+\frac{\paren{\paren{2|\domClabel|\sqrt{\ln{|\domClabel|}}+2}{{\sqrt{\frac{T\cdot \paren{2d\ln{\frac{eT}{d}}+\ln{\frac{2}{\delta}}}}{{\fixremoved{\max}\{\minpgap{T},\fixremoved{\sqrt{1/{T}}}\}}}}}}+\tilde{\Loss}_{T,*}}\paren{\log_{|\domClabel|}{\paren{T|\domClabel|}}}}{|\domClabel|},\\
\end{flalign*}

since the second term dominates the upper bound, we have
\begin{align*}
{O}\paren{\expct{\sum_{t=1}^TU_t}}&={O}\paren{
\frac{\paren{{{\sqrt{\frac{T\cdot \paren{2d\ln{\frac{eT}{d}}+\ln{\frac{2}{\delta}}}}{{\fixremoved{\max}\{\minpgap{T},\fixremoved{\sqrt{1/{T}}}\}}}}}}+\tilde{\Loss}_{T,*}}\paren{\ln\paren{T}}}{|\domClabel|\ln{|\domClabel|}}}\\
&\stackrel{\paren{a}}{=}\fixremoved{{O}\paren{
\frac{\paren{{{\sqrt{\frac{T\cdot \paren{2d\ln{\frac{eT}{d}}+\ln{\frac{2}{\delta}}}}{{\fixremoved{\max}\{\minpgap{T},\fixremoved{\sqrt{1/{T}}}\}}}}}}+\tilde{\Loss}_{T,*}}\paren{\ln\paren{T}}}{\numClabel\ln{\numClabel}}},}
\end{align*}

\fixremoved{where step (a) is by applying $\numClabel=|\domClabel|$.}

\end{proof}
















==> supp_related_works.tex <==
\section{Related Work}\label{app:related_work}
\paragraph{Contextual bandits.} Classical bandit algorithms%
(e.g., EXP3 \citep{auer2002nonstochastic} or UCB \citep{auer2002finite}) aim to find the best action(s) achieving the minimal regret through a sequence of actions. When side information (e.g. user profile for recommender systems or environmental context for experimental design) is available at each round, many bandit algorithms can be lifted to the contextual setting: For example, EXP4 and its variants \citep{auer2002nonstochastic,beygelzimer2011contextual,neu2015explore} consider the bandit setting with expert advice: At each round, experts announce their predictions of which actions are the most promising for the given context, and the goal is to construct a expect selection policy that competes with the best expert from hindsight. Note that in bandit problems, the learner only gets to observe the reward for each action taken. {In contrast, for the online model selection problem considered in this work---where an action corresponds to choosing a model to make prediction on an incoming data point---we get to see the loss/reward of \textit{all} models on the labeled data point.} {By utilizing the information from unchosen arms, it could reduce the cumulative regret in a non-trival scale.}
{In this regard, our work aligns more closely with online learning with \textit{full information} setting, where the learner has access to the loss of all the arms at each round (e.g. as considered in the Hedge algorithm \citep{freund1997decision,burtini2015survey,cesa2006prediction,hoi2021online}).}

\paragraph{Online learning with full information.} A clear distinction between our work and online learning is that %
we assume the labels of the online data stream are not readily available but can be acquired at each round with a cost. In addition, the learner only observes the loss incurred by all models on a data point when it decides to query its label. In contrast, in the canonical online learning setting, labels arrive with the data and one gets to observe the loss of all candidate models at each round. Similar setting also applies to other online learning problems, such as online boosting or bagging. %
A related work to ours is online learning with label-efficient prediction \citep{cesa2005minimizing}, which proposes an online learning algorithm with matching upper and lower bounds on the regret. However, they consider a fixed query probability that leads to a linear query complexity. Our algorithm, inspired by uncertainty sampling in active learning, achieves an improved query complexity with the adaptive query strategy while maintaining a comparable regret.






\paragraph{Stream-based Active learning.}%
Active learning aims to achieve a target learning performance with fewer training examples \citep{settles2009active}. 
The active learning framework closest to our setting is query-by-committee (QBC) \citep{seung1992query}, in particular under the stream-based setting %
\citep{loy2012stream,ho2008query}. QBC maintains a committee of hypotheses; each committee member votes on the label of an instance, and the instances with the maximal disagreement among the committee are considered the most informative labels. Note that existing stream-based QBC algorithms are designed and analyzed assuming i.i.d. data streams. In comparison, our work uses a different query strategy as well as a novel model recommendation strategy, which also applies to the adversarial setting.

\paragraph{Active model selection.} Active model selection captures a broad class of problems where model evaluations are expensive, either  due to (1) the cost of evaluating (or ``probing'') a model, or (2) the cost of annotating a training example. 
Existing works under the former setting  \citep{madani2012active,santana2020contextual} {and online setting \citep{cutkosky2021dynamic,shukla2019adaptive}} often ignore context information and data annotation cost, and only consider \emph{partial} feedback on the models being evaluated/ probed on i.i.d. data. The goal is to identify the best model with as few model probes as possible. %
This is quite different from our problem setting which considers the full information setting as well as non-negligible data annotation cost. 
{
\citep{van2018almost} proposes that the optimal model choice is influenced by the sample size rather than any individual sample feature.
\citep{li2020finding} addresses the active model selection problem, however both works do not adopt a stream-based approach.}
For the later, apart from \citet{karimi2021online}, {an online contextual-free model selection work}, as shown in \tabref{tab:alg:characteristics}, most existing works assume a pool-based setting where the learner can choose among the pool of unlabeled data \citep{sugiyama2008batch,madani2012active,sawade2012,sawade2010active,ali2014active,gardner2015bayesian,zhang2014beyond,leite2010active}, and the goal is to identify the best model with a minimal set of labels. 


















\clearpage


